Parameter estimation of structural dynamics with neural operators enabled surrogate modeling

Parameter estimation in structural dynamics generally involves inferring the values of physical, geometric, or even customized parameters based on first principles or expert knowledge, which is challenging for complex structural systems. In this work, we present a unified deep learning-based framework for parameterization, forward modeling, and inverse modeling of structural dynamics. The parameterization is flexible and can be user-defined, including physical and/or non-physical (customized) parameters. In the forward modeling, we train a neural operator for response prediction -- forming a surrogate model, which leverages the defined system parameters and excitation forces as inputs to the model. The inverse modeling focuses on estimating system parameters. In particular, the learned forward surrogate model (which is differentiable) is utilized for preliminary parameter estimation via gradient-based optimization; to further boost the parameter estimation, we introduce a neural refinement method to mitigate ill-posed problems, which often occur in the former. The framework's effectiveness is verified numerically and experimentally, in both interpolation and extrapolation cases, indicating its capability to capture intrinsic dynamics of structural systems from both forward and inverse perspectives. Moreover, the framework's flexibility is expected to support a wide range of applications, including surrogate modeling, structural identification, damage detection, and inverse design of structural systems.

==> content/preliminaries.tex <==
\subsection{Mappings in structural dynamics}
\label{pre:structural}

Consider a \textit{structural dynamical system}, as presented in Figure~\ref{fig:sd}, which is characterized by the relationship between the input functions and output functions defined as follows: 
\begin{align}
    y(t) = \mathcal{M} \left(\boldsymbol{\mu}, f(t) \right).
    \label{eq:forward}
\end{align}
Here, $\mathbf{\mu} = \{\mu_1, \mu_2, ...\}$ represents the system's parameters, and $f(t)$ denotes the external excitation force function, and $y(t)$ is the system's response function.  
The parameters $\mu$ can be structural physical quantities, such as mass, stiffness, and damping coefficients or non-physical (abstract) quantities like component shape, damage serverity, or other relevant characteristics depending on the application.
The operator $\mathcal{M}$ maps the system parameters space and excitation force space to the dynamic response space, typically involving solving the intrinsic dynamics of the system, often through convolution operations.
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{structural_dynamics_2.eps}
    \caption{Structural dynamics is defined by the mapping of input functions and output functions.}
    \label{fig:sd}
\end{figure}


This study focuses on two key aspects of structural dynamics modeling:
\begin{itemize}
    \item \textit{Forward modeling}: The mapping from the system's parameters and excitation force to the dynamic response. 
    Specifically, we focuses on the response prediction when the system's parameters are changed or unknown.
    \item \textit{Inverse modeling}: The estimation of the system's parameters from the dynamic response and excitation force.
    In particular, we also aim to estimate the changed or unknown system parameters from the dynamic response and excitation force.
\end{itemize}
Although force identification is another aspect of inverse modeling, it is not considered in our current attempt.
The primary objective of this research is to develop a unified data-driven framework that addresses both response prediction (forward modeling) and parameter estimation (inverse modeling) in structural dynamics.



\subsection{DeepONet}
Recently, considerable efforts have been made to develop neural networks that approximate operators for solving partial differential equations (PDEs). 
Lu et al.~\cite{lu2021learning} proposes the deep neural operator (DeepONet), which employs a branch-trunk architecture that is based on the universal approximation theorem for the operator~\cite{chen1995universal}.

In the operator setting of the vanilla DeepONet~\cite{lu2021learning,zhu2023reliable}, two function spaces are considered. 
Let a function space $\mathcal{U}$, which consists of functions $u$ defined on the domain $D \subset \mathbb{R}^d$:
\begin{equation}
    u: D \ni x \mapsto u(x) \in \mathbb{R}, 
\end{equation}
, and another function space $\mathcal{V}$, with functions $v$ defined on a domain $D^{\prime} \subset \mathbb{R}^{d^{\prime}} $:
\begin{equation}
    v: D^{\prime} \ni \xi \mapsto v(\xi) \in \mathbb{R},
\end{equation}
where $x$, $\xi$ are the evaluation points in $\mathcal{D}^\prime$, $\mathcal{D}$, respectively. These evaluation points can be identical or distinct according to application settings~\cite{lu2022comprehensive}. 
Then, the mapping between the function space $\mathcal{U}$ and the function $\mathcal{V}$ is defined by an operator $\mathcal{G}$ as follows:
\begin{equation}
    \mathcal{G}: \mathcal{U} \rightarrow \mathcal{V}, \quad u \mapsto v .
\end{equation}

The motivation of DeepONet is to approximate the operator $\mathcal{G}$ via the neural network architectures and optimization techniques. 
As illustrated in Figure~\ref{fig:deeponet}, it includes two components: the branch net and the trunk net. 
For $m$ scattered evaluation point $\left\{x_1, x_2, \ldots, x_m\right\}$ in $D$, the branch net takes the v at these evaluation points as input and outputs the $\left[b_1(v), b_2(v), \ldots, b_p(v)\right]$, where $p$ is the number of neurons. The trunk net takes the $\xi$ as input and outputs $\left[t_1(\xi), t_2(\xi), \ldots, t_p(\xi)\right]$.

The branch net encodes functions from $\mathcal{U}$ as input, while the trunk net evaluates the functions from $\mathcal{Y}$ at specific output locations. 
The forward process of DeepONet is as: 
\begin{align}
    & \hat{\mathcal{G}}(u)(\xi) = \sum_{k=1}^{p} b_{k}(u) \times t_{k}(\xi), \\
    & |\mathcal{G}(u)(\xi)-\hat{\mathcal{G}}(u)(\xi)|<\epsilon,
\end{align}
where $b_k$ and $t_k$ are the $k$-th dimensions of the outputs of the branch and trunk nets, respectively, and $\epsilon$ represents a small error tolerance.
\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{deeponets.eps}
    \caption{The illustrations of vanilla DeepONet and Enhanced DeepONet for structural dynamics.}
    \label{fig:deeponet}
\end{figure}
Similar to neural networks, neural operators are trained via the empirical risk minimization strategy. Given architecture and training data, the neural operator's parameters are optimized by stochastic gradient descent. 







